Singly generated operator algebras satisfying weakened versions of amenability

We construct a singly generated subalgebra of ${\mathcal K}({\mathcal H})$ which is non-amenable, yet is boundedly approximately contractible. The example embeds into a homogeneous von Neumann algebra. We also observe that there are singly generated, biflat subalgebras of finite Type I von Neumann algebras, which are not amenable (and hence are not isomorphic to C*-algebras). Such an example can be used to show that a certain extension property for commutative operator algebras, which is shown in arXiv:1012.4259 to follow from amenability, does not necessarily imply amenability.

==> bac-oa_mac2b.tex <==

%-------------
\RequirePackage{amsmath,amssymb,amsfonts,amscd}
\usepackage{hyperref}
\usepackage[usenames]{color}


%----- YC FORMATTING -------
%----- CHANGE WHEN TYPESETTING THE VOLUME?

%% MARGINS ETC
\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-60mm}
\setlength{\oddsidemargin}{5mm}
\setlength{\evensidemargin}{5mm}
\setlength{\topmargin}{-2mm}
\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-71mm}

%% Emphasis and definitions
\renewcommand{\emph}[1]{{\sl #1}\/} % use slanted font for emphasis
\newcommand{\dt}[1]{{\it #1}\/}
% Rem this out
\renewcommand{\dt}[1]{\textcolor{Bittersweet}{\sf#1}}

%% THEOREMS
\RequirePackage{amsthm}   %Inbuilt environments for defns etc

\newcounter{pulse}[section]
\numberwithin{pulse}{section}  % all thms, etc set from pulse


%Styles for theorems, definitions, remarks
\newcommand{\thf}{\sc} % alias for theorem heading font

%-Theorems
\theoremstyle{plain}
\newtheorem{thm}[pulse]{\thf Theorem}
\newtheorem{prop}[pulse]{\thf Proposition}
\newtheorem{lem}[pulse]{\thf Lemma}
\newtheorem{cor}[pulse]{\thf Corollary}
%-Definitions
\theoremstyle{definition}
\newtheorem{dfn}[pulse]{\thf Definition}
%-Remarks
\theoremstyle{remark}
\newtheorem{rem}[pulse]{\thf Remark}

%----- END YC FORMATTING



%% Gumpf
\newcommand{\contact}{%
Department of Mathematics and Statistics\\
McLean Hall\\
University of Saskatchewan\\
106 Wiggins Road, Saskatoon, SK\\
Canada, S7N 5E6
}

%%Grammar
\newcommand{\st}{\,:\,}
\newcommand{\defeq}{:=}
\newcommand{\sid}{\operatorname{\sf id}}  % generic notation for identity map

% upright roman numerals in numbered lists, we need to force this if in an italic environment
\newenvironment{YCnum}{%
\begin{enumerate}
\renewcommand{\labelenumi}{{\rm(\roman{enumi})}}
\renewcommand{\theenumi}{{\rm(\roman{enumi})}}
}{\end{enumerate}\ignorespacesafterend}


%%Personal preference and fundamentals
\newcommand{\iso}{\cong}
\newcommand{\tp}{\mathop{\otimes}\nolimits}
\newcommand{\id}[1][]{{\sf 1}_{#1}} % identity of group, algebra, object in category
\newcommand{\wstar}{\ensuremath{{\rm w}^*}}
\newcommand{\fu}[1]{{#1}^{\sharp}}    % forced unitisation
                % Helemskii denotes this by A_+, etc.

\newcommand{\tr}{\operatorname{Tr}} % matrix trace
\newcommand{\spec}{\operatorname{sp}} % spectrum
\newcommand{\pair}[2]{\langle{#1},\,{#2}\rangle}

\newcommand{\ptp}{\mathop{\widehat{\otimes}}\nolimits} % projective tensor product

% Abs value, norm
\newcommand{\abs}[1]{\vert{#1}\vert}
\newcommand{\Abs}[1]{\left\vert{#1}\right\vert}
\newcommand{\norm}[1]{\Vert{#1}\Vert}
\newcommand{\Norm}[1]{\left\Vert{#1}\right\Vert}
\newcommand{\clin}{\overline{\rm lin}} %closed linear span

%-Banach spaces
\newcommand{\Bdd}{{\mathcal B}}
\newcommand{\lpsum}[1]{\overset{({#1})}{\bigoplus}}

%Rings, fields
\newcommand{\Cplx}{\mathbb C}
\newcommand{\Nat}{\mathbb N}
\newcommand{\Rat}{\mathbb Q}
\newcommand{\Real}{\mathbb R}
\newcommand{\Zahl}{\mathbb Z}

\newcommand{\VN}{\operatorname{VN}}
\newcommand{\Cst}{\operatorname{C}^*}


%---------------

\newcommand{\fA}{{\mathfrak A}}
\newcommand{\fB}{{\mathfrak B}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\Cpct}{{\mathcal K}}
\newcommand{\sG}{{\mathsf G}}

\newcommand{\Z}{{\mathbb Z}}

\newcommand{\al}{\alpha}
\newcommand{\kp}{\kappa}
\newcommand{\lm}{\lambda}
\newcommand{\om}{\omega}
\newcommand{\ip}[2]{\langle #1 , #2\rangle}
\newcommand{\lin}{\operatorname{lin}}
\newcommand{\ran}{\operatorname{ran}}
\newcommand{\ad}{\operatorname{ad}}
\newcommand{\Mat}{{\mathbb M}}

\newcommand{\bac}{boundedly approximately contractible}
\newcommand{\ac}{approximately contractible}
\newcommand{\mbad}{multiplier-bounded approximate diagonal}

\newcommand{\snorm}[1]{\norm{#1}_{(1)}} % unnormalized trace-class norm
\newcommand{\sNorm}[1]{\Norm{#1}_{(1)}} % unnormalized trace-class norm

\newcommand{\typone}{Type~${\rm I}$}
\newcommand{\twoone}{{\rm II}_1} % II_1
\newcommand{\typtwoone}{Type~$\twoone$}


